Localization length index in a Chalker-Coddington model: a numerical study

We calculated numerically the localization length index $\nu$ for the Chalker-Coddington model of the plateau-plateau transitions in the quantum Hall effect. By taking into account finite size effects we have obtained $\nu = 2.593 \pm 0.0297$. The calculations were carried out by two different programs that produced close results, each one within the error bars of the other. We also checked the possibility of logarithmic corrections to finite size effects and found, that they come with much larger error bars for $\nu$.

==> CClattice.tex <==
\begin{tikzpicture}
	[lattice matrix/.style={
		row sep=0.55cm, 
		column sep=0.55cm,
%		execute at begin cell=\node{}\bgroup,
%		execute at end cell=\egroup;,%
		matrix of math nodes,
		execute at empty cell=\node[coordinate]{};,
	},
 	>=stealth']%,
% 	thick]


\matrix(M)[lattice matrix]{
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
 		 &  &  &  &   &  &  &  &   &  &  &  &  & & \\
	};

\foreach \aa / \ab / \ac / \ad / \ae in {1/2/3/4/5, 5/6/7/8/9}
		\foreach \ba / \bb / \bc / \bd / \be in {1/2/3/4/5, 5/6/7/8/9, 9/10/11/12/13}
			{
				\draw (M-\ab-\ba)--(M-\ab-\bc);
				\draw[->] (M-\ab-\bb)--(M-\aa-\bb);
				\draw (M-\ab-\bb)--(M-\ac-\bb);
				\draw[->](M-\ab-\bb)--(M-\ab-\bc);
				\draw[->,dashed] (M-\ac-\ba)--(M-\ab-\bb);
				\draw[->,dashed] (M-\ab-\bb)--(M-\aa-\bc);
				\draw (M-\ab-\bc)--(M-\ab-\bd);
				\draw(M-\ab-\bd)--(M-\aa-\bd);
				\draw[->](M-\ab-\bd)--(M-\ab-\be);
				\draw[->](M-\ab-\bd)--(M-\ac-\bd);
				\draw[->,dashed](M-\aa-\bc)--(M-\ab-\bd);
				\draw[->,dashed](M-\ab-\bd)--(M-\ac-\be);
								
				\draw[->](M-\ad-\bb)--(M-\ad-\ba);
				\draw[->](M-\ad-\bb)--(M-\ac-\bb);
				\draw (M-\ad-\bb)--(M-\ae-\bb);
				\draw (M-\ad-\bb)--(M-\ad-\bc);
				\draw[->,dashed](M-\ad-\bb)--(M-\ac-\ba);
				\draw[->,dashed](M-\ae-\bc)--(M-\ad-\bb);
				\draw[->](M-\ad-\bd)--(M-\ad-\bc);
				\draw(M-\ad-\bd)--(M-\ad-\be);
				\draw(M-\ad-\bd)--(M-\ac-\bd);
				\draw[->](M-\ad-\bd)--(M-\ae-\bd);
				\draw[->,dashed](M-\ad-\bd)--(M-\ae-\bc);
				\draw[->,dashed](M-\ac-\be)--(M-\ad-\bd);

				\node[above] at (M-\ab-\bc) {t};
				\node[above] at (M-\ab-\be) {r};
				\node[left] at (M-\ac-\bb) {t};
				\node[right] at (M-\ac-\bd) {t};
				\node[below] at (M-\ad-\bc) {t};
				\node[below] at (M-\ad-\be) {r};
%				\node[right] at (M-\ae-\bb) {r};
%				\node[left] at (M-\ae-\bd) {r};
			};
			\foreach \xa / \xb in {2/4,6/8,10/12}{
				\node[right] at (M-5-\xa) {r};
				\node[left] at (M-5-\xb) {r};
			};
			
			\foreach \y / \ly in {8/2j-1,6/2j,4/2j+1,2/2j+2}
				\node[left] at (M-\y-1) {\textsl{\ly}};
%			\foreach \x / \lx in{2/t,4/t+1,6/t+2,8/t+3,10/t+4,12/t+5}
%				\node[below] at (M-9-\x){\textsl{\lx}};
			\foreach \x in {3,7,11}
				\node[below] at (M-9-\x){$M_1$};
			\foreach \x in {5,9}
				\node[below] at (M-9-\x){$M_2$};
\end{tikzpicture}

==> bin_plot2.tex <==
\begin{tikzpicture}
	\begin{axis}[
			width=\columnwidth,
			height=6.5cm,
			/pgf/number format/precision=3,
			axis x line=bottom,
			axis y line=left,
			xlabel=$\gamma$,
			ylabel=points per interval,
			mark options={mark=none},
			enlarge x limits=auto,
		]
		\addplot+[ybar, bar width=3.6pt, fill, opacity=0.5] table[x=x,y=bin_num] {bin_plot2.dat} \closedcycle;
		\addplot+[smooth] table[x=x,y=gauss] {bin_plot2.dat};
	\end{axis}
\end{tikzpicture}

==> fit_plot.tex <==
\begin{tikzpicture}
	\begin{axis}[
			width=\columnwidth,
%			height=6cm,
			/pgf/number format/precision=3,
			axis x line=bottom,
			axis y line=middle,
			xlabel=$x$,
			ylabel=$M\Gamma$,
			ylabel style={at={(-0.13,0.44)},rotate=90},			
			enlarge x limits=auto,
			mark options={mark=x},
			/pgfplots/error bars/error mark=|,
			/pgfplots/error bars/error mark options={scale=1.5},
			/pgfplots/error bars/error bar style={solid},
			legend style={at={(0.5, 1)}},
		]

		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b20] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b30] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b40] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b50] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b60] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b70] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b80] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b100] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b120] {plotdat.dat};
		\addplot+[smooth,mark options={mark=none}] table[x=X,y=b140] {plotdat.dat};

		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x20,y=g20,y error=dg20]{outputdat20.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x30,y=g30,y error=dg30]{outputdat30.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x40,y=g40,y error=dg40]{outputdat40.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x50,y=g50,y error=dg50]{outputdat50.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x60,y=g60,y error=dg60]{outputdat60.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x70,y=g70,y error=dg70]{outputdat70.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x80,y=g80,y error=dg80]{outputdat80.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x100,y=g100,y error=dg100]{outputdat100.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x120,y=g120,y error=dg120]{outputdat120.dat};
		\addplot plot[only marks, error bars/.cd, y dir=both,y explicit]
			table[x=x140,y=g140,y error=dg140]{outputdat140.dat};

 		\legend{20 blocks, 30 blocks, 40 blocks, 50 blocks, 60 blocks, 70 blocks, 80 blocks, 100 blocks, 120 blocks, 140 blocks}

	\end{axis}
\end{tikzpicture}
